Documentation Matters: Human-Centered AI System to Assist Data Science Code Documentation in Computational Notebooks

Computational notebooks allow data scientists to express their ideas through a combination of code and documentation. However, data scientists often pay attention only to the code, and neglect creating or updating their documentation during quick iterations. Inspired by human documentation practices learned from 80 highly-voted Kaggle notebooks, we design and implement Themisto, an automated documentation generation system to explore how human-centered AI systems can support human data scientists in the machine learning code documentation scenario. Themisto facilitates the creation of documentation via three approaches: a deep-learning-based approach to generate documentation for source code, a query-based approach to retrieve online API documentation for source code, and a user prompt approach to nudge users to write documentation. We evaluated Themisto in a within-subjects experiment with 24 data science practitioners, and found that automated documentation generation techniques reduced the time for writing documentation, reminded participants to document code they would have ignored, and improved participants' satisfaction with their computational notebook.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> review/changes.tex <==
## abstract and title
- remove framing around human-AI collaboration, keep them only in the discussion (R2)

## related work
-  Lau et al. paper could serve to structure 2.1 as it provides a good overview of the design space of notebooks. This could help position more clearly the work done with Themisto. Indeed improving explanations in computational notebooks can be done in many ways, and improve markdown cells is only one aspect. This would open up the discussion to other "intelligent" strategies that could be put into place to support explanations in notebooks. Many strategies interact with markdown comments: breaking-down cells could help with more straightforward comments, supporting cell re-ordering could help with better headers/structrue, facilitating cell folding could help surface important markdown cells (see Rule et al. CSCW'18), or support for history (Kery et al.) and branching (Wood et al.) would also help create simpler or richer narratives. (R2)
- In addition to this, I think that Woods et al. "Design Exposition with Literate Visualization" who also be worth discussing as it proposes interesting profiles on rather than a "one size fits all" approach to how literate programming should be. (R2)
- - Ln 173 “But those winning solutions are often not the most voted ones, as community members voted on readability and completeness of the computational narrative.” I don’t know if this characterization is entirely accurate. Do we know for sure that users are voting based on readability or completeness? A missing part of this characterization is that shared notebooks on Kaggle don’t all share the same purpose. Some are collaborative efforts shared during an active content [Tausczik & Wang 2017], some are tutorials written by the Kaggle platform, and some are computational narratives/tutorials/analysis walkthroughs written by members of the community **presumably because** even if you cannot win competitions, you can “win at” and gain ranking points and status, by writing popular notebooks ( see https://www.kaggle.com/progression). Tausczik & Wang found that notebooks written by higher-status members of the community or notebooks that are *more similar* to most other notebooks are more likely to get forked/edited by others. There may be a homogeneity affect going on in the sample here, that high ranked notebooks tend to follow certain style or technology conventions as other high ranked notebooks. I would like just a bit more detailed characterization of the Kaggle platform, because it really does affect what kind of data the authors are sampling in this study.
   - Relevant citation: Tausczik, Yla, and Ping Wang. "To share, or not to share? Community-level collaboration in open innovation contests." Proceedings of the ACM on Human-Computer Interaction 1, no. CSCW (2017): 1-23. (R3)
   
- Ln 180 “However, writing documentation itself is a time-consuming task. And that is why documentation practices in open source communities are widely perceived to be of low quality, due in part to low levels of intrinsic enjoyment for doing documentation work” Missing some of the key issues with software documentation: 1) documentation easily gets out-of-date and is expensive to keep updated over time, 2) it’s not clear how much documentation is needed, and 3) not all documentation is equally useful.
   - Relevant citation: Aghajani, Emad, Csaba Nagy, Olga Lucero Vega-Márquez, Mario Linares-Vásquez, Laura Moreno, Gabriele Bavota, and Michele Lanza. "Software documentation issues unveiled." In 2019 IEEE/ACM 41st International Conference on Software Engineering (ICSE), pp. 1199-1210. IEEE, 2019. (R3)
   
   
## formative study

## system design

- Raises two points regarding the implementation of the tool: how much does the notebooks used for the training shape the quality/relevance of the outputs? What were the competitions used? how was the dataset assembled and to what extent outputs differ from inputs (i.e., would some output infringe on copyright ?).  This is also relevant to the evaluation as it is unclear whether the two different data-science problems are related to the training data, as this would likely influence the results. (R2)

- Also raises concerns regarding a generalizability argument for the selected corpus. Why do we expect that beginner tutorial notebook documentation is representative of documentation in general data science notebooks used in industry or research? “Kaggle is an excellent source… but are you going to get a sample bias that this is a platform focused on education and learning data science? I wonder if Kaggle notebooks may be more like tutorials than, for instance, notebooks published with papers?” Do we know for sure that users are voting based on readability or completeness? (R3)

## evaluation

- (done) requests clarifications regarding the experimental task used to evaluate the tool. Was the scope and duration of the task sufficient? It would be beneficial to elaborate on the rationale for the task.

(done) Also, the scope of the notebook (9 cells) is limited. Please clarify whether winning Kaggle notebooks (which were used as a base for this notebook) are representative of realistic notebooks? (R1)

- Requests clarifications regarding the method: Why have participants evaluate their own notebook rather than a peer grading situation or only the independent grader situation? Do the expert graders use the same rubric that participants used for themselves? How do these two grading schemes match up? (R3)

## discussion

- Suggests ways to deepen the discussion including:
(1) human-ai collaboration for documentation, (2) using the proposed approach to support better documentation beyond the generation of markdown, (3) future functionality and evaluation of Themisto. (R2)

- In addition, R1 asks for the authors thoughts on how Themisto would impact user performance after using it for an extended period of time (e.g. for several weeks)? I would like to see this deliberated as part of the Discussion. (R1)

## appendix

- (done) Would like to see examples of co-created documentation. What did the machine generate and what did the human add to it or how did they edit it?  Also, raises several questions regarding the results that should be addressed. (R3)


## figures, tables
- (done) Table 2 is never referenced from the text. (R1)

- (done) Table 4 doesn't seem the best way to present all this data (or at least it makes it feel under-sold) E.g., a bar chart with standard error bars for task time of each task comparing the treatments I think would better highlight the big differences. There is a lot of good stuff here and breaking it up visually I think would better convey the differences, though I'm sure there is some concern about making the paper even longer. (R1)

- (done) I like Figure 7 except that it omits several of the questionnaire questions. Where are those results? (R1)

- (done) Figure 5 is very helpful. Only minor suggestion is to increase the font sizes. (R1)

- (done) Some of the text in figures is small and can be made bigger. For example, the numbers in Figure 2, the cells in Figure 5, and the text in Figure 6. (R1)

- Table 2 could be complemented by a plot showing the distribution of markdown cells. (R2)

- (done) Fig 2. Please label the red column and the blue column of plots, I had to read the figure caption several times to figure out red is Kaggle and blue is GitHub. Additionally, there are these tiny faint labels inside of the bottom 3 graphs that are redundant with the outside labels… maybe get rid of those. Finally, please make the x axis scale numbers a bit bigger for legibility, the same font size as the left labels ideally. (R3)

- Fig 5. Nice figure! I now see that “tokenize” in step 3 is *not* tokenize in the programming languages sense, but tokenize as in convert to an index in a dictionary. However, I still don’t fully see how the AST was tokenized: based on the node type name like “Assign?” Or something else? (R3)

- (done) Fig 6. The code is way too small to read. I understand how hard it is to make figures showing code, but the 3 column layout here might not be possible. Perhaps 3 rows of A, B, C instead? Better extra-large code than tiny illegible code. (R3)

- (done) Fig 7. There is one disagree or strongly disagree for each question, how intriguing. Was it all the same person who just happened to really hate the tool? A little context would be helpful in the caption. (R3)


## Others (done)
- Footnotes 11 and 12 seem to be important details that they should be in the paragraph. (R1)
- P2 L53/54 : prove the statement or tone it down. Some analysts do work on notebooks collaboratively, the (R2)
- P4 L199 : guidlines -> guidelines (R2)
- P5 L353 : practice is not the right term here. (R2)
- P5 L355 : stoped -> stopped (R2)
- P14 User Evaluation : were you expecting to see an effect of gender on the performance? if not, why report it? (R2)
- Ln. 373 “We replicated tne notebook descriptive analysis” typo (R3)


==> review/review.tex <==
===============================================
Any reviews entered for this paper, will appear below this point.
This is timely and important work with the advent of automation for coding and data science. Computational notebooks are increasingly of interest for the CHI community (and beyond).

**
This paper presents Themisto, a tool documentation generation, which uses an approach that combines machine learning, retrieval of online API documentation, and eliciting documentation from users. The authors present findings from a formative study on documentation practices and results from the evaluation of Themisto.

Overall, the reviewers agree that this paper is well written, the research is motivated and relevant, and that the methodology is adequate.  Having read the manuscript myself, I echo the reviewers’ assessments. With some (relatively minor) changes, the paper has a high likelihood of acceptance.

Following, I summarized the main reviewers’ comments, please read the individual reviews carefully as each of the reviewers also make minor points (not summarized here) that should be addressed in the submission:

R1:
requests clarifications regarding the experimental task used to evaluate the tool. Was the scope and duration of the task sufficient? It would be beneficial to elaborate on the rationale for the task.

Also, the scope of the notebook (9 cells) is limited. Please clarify whether winning Kaggle notebooks (which were used as a base for this notebook) are representative of realistic notebooks?

In addition, R1 asks for the authors thoughts on how Themisto would impact user performance after using it for an extended period of time (e.g. for several weeks)? I would like to see this deliberated as part of the Discussion.

Suggests breaking Table 4 into several visual components, E.g., a bar chart with standard error bars for task time of each task comparing the treatments. I’d suggest charting the task time, while leaving the rest of the data in the table.

Update or clarify why Figure 7 presents only some of the results from the post-task questionnaire.

R2:
Requests to remove reference to human-AI collaboration and describe the contribution more precisely. “I was surprised by the discrepancy between the positioning around human-AI collaboration, and the actual contribution of the paper. The topic is quite popular at the moment, but there is no human-AI _collaboration_ in Themisto. A prompt/auto-filling that can be corrected by users can hardly fall in a collaboration category.”

Suggests that the initial framing of the contribution and the discussion would benefit from engaging more deeply with the possibilities of improving narration in notebooks, and how intelligent strategies could be used not only for md cells. R2 provided references for relevant related work.

Requests clarification on naming categories in the formative study, as well as to discuss and elaborate on the limitations of the corpus.

Raises two points regarding the implementation of the tool: how much does the notebooks used for the training shape the quality/relevance of the outputs? What were the competitions used? how was the dataset assembled and to what extent outputs differ from inputs (i.e., would some output infringe on copyright ?).  This is also relevant to the evaluation as it is unclear whether the two different data-science problems are related to the training data, as this would likely influence the results.  

Suggests ways to deepen the discussion including:
(1) human-ai collaboration for documentation, (2) using the proposed approach to support better documentation beyond the generation of markdown, (3) future functionality and evaluation of Themisto.


R3

Also raises concerns regarding a generalizability argument for the selected corpus. Why do we expect that beginner tutorial notebook documentation is representative of documentation in general data science notebooks used in industry or research? “Kaggle is an excellent source… but are you going to get a sample bias that this is a platform focused on education and learning data science? I wonder if Kaggle notebooks may be more like tutorials than, for instance, notebooks published with papers?” Do we know for sure that users are voting based on readability or completeness?

Related to this point, R3 would like to see a more focused framing of this paper and an argument for generalization and representative sample: “are beginner tutorial notebooks really what we are aiming for? I could certainly be convinced that tutorial notebooks are the epitome of a good computational narrative, but that argument is currently missing from the story. Beginner tutorial is a really specific flavor of documentation, but the paper is presenting this sample as generalizable and representative of all documentation? Or all documentation we should aim for?”

Proposes several ways to deepen the engagement with related work (including additional references).

Related to implementation of Themisto – “how does Themisto choose between the 3 approaches? Does it choose between them at this point as a prototype? Does Themisto suggest documentation for *every* cell, or are there cases in which it decides to leave a code cell as-is?”

Suggests improvement  for Figures 2, 6

Requests clarifications regarding the method: Why have participants evaluate their own notebook rather than a peer grading situation or only the independent grader situation? Do the expert graders use the same rubric that participants used for themselves? How do these two grading schemes match up?

Would like to see examples of co-created documentation. What did the machine generate and what did the human add to it or how did they edit it?  Also, raises several questions regarding the results that should be addressed.


In conclusion, all reviewers (including this AE) view this paper as timely, relevant, and well written, and value the contributions of both the formative study and the tool and its evaluation. The reviewers provided detailed feedback, which includes concerns which need to be addressed through discussion and clarifications, as well as suggestions for improvement. To summarize: There are two critical issues which need to be addressed by the authors:

1. Questions and concerns regarding the ecological validity of the study, these should be addressed in the Method. As well as discussion of the limitations of the corpus used in the formative study in terms of its generalizability and whether the sample is indeed representative of the broader data science notebooks space.

2. Presenting Themisto as an example of human-AI collaboration seems exaggerated for the described interaction (prompts) and review of auto-generated text. Please remove reference to human-AI collaboration (including from abstract and title) and describe the contribution more precisely. The results and discussion should provide evidence for documentation created by both humans and Themisto.


I look forward to reading the revised manuscript. Following you can find the reviews.

**
Referee: 1

Recommendation: Needs Minor Revision

Comments:
(There are no comments.)

Additional Questions:
The Review:  
This paper contributes Themisto, a tool for assisting with documentation generation using a machine learning approach, retrieving info from online documentation, and eliciting more documentation from users. Also presented are the results of a formative study on documentation practices and the results from evaluating Themisto with a comparative lab study. The evaluation found that Themisto reduced the time for data scientists to create documentation, reminded them to document code they would have ignored, and improved their satisfaction with their notebooks.

Computational notebooks are of huge interest, within the CHI community and beyond, and being able to efficiently clean and organize notebooks seems to be a consistent struggle for everyone (including myself!).

In fact, this paper looks like a great HCI paper. It is grounded in a relatable problem, has a formative study motivating the tool design, has an evaluation, and presents a novel system with a clear explanation of the user interface and internal workflow. Moreover, the paper is well written and has a nice Related Work section (the code summarization section was particularly helpful). There is *a lot* of content in this paper.

While I don't have any major concerns about the paper, there are a number of issues that I'd like clarified. I think doing so could make this already good paper even better. They are as follows, in a rough order of importance:

- 9 cells for the notebooks in the evaluation study seems very small (especially when referring back to Figure 2). The footnote says they are "based on" two winning Kaggle notebooks, but are winning Kaggle notebooks representative of realistic notebooks? If they are only based on them then it opens three more questions: (1) Who changed them? (2) By how much? (3) What kind of changes?

- 12 minutes per task in the evaluation seems a bit short. Was this really enough time for users to be effective using Themisto? The footnote says that a pilot study showed that participants completed the tasks within 10 minutes. Does this mean the task is too simple/artificial?

- Footnotes 11 and 12 seem to be important details that they should be in the paragraph.

- Table 2 is never referenced from the text.

- Any thoughts on how one's performance might look after using Themisto for several weeks? I don't expect another study to be run for this paper, simply asking for the author's opinion. It could make for interesting discussion. Only having a 1 minute demo seems so short.

- Thank you for the examples in the appendix. Very helpful.

- Table 4 doesn't seem the best way to present all this data (or at least it makes it feel under-sold) E.g., a bar chart with standard error bars for task time of each task comparing the treatments I think would better highlight the big differences. There is a lot of good stuff here and breaking it up visually I think would better convey the differences, though I'm sure there is some concern about making the paper even longer.

- I like Figure 7 except that it omits several of the questionnaire questions. Where are those results?

- The design implications are awesome!

- The UI and implementation details are clear, good job!

- I think that the negative feedback from participants about specific methods, either the query or deep-learning approach, are particularly interesting for future work and not a negative on Themisto specifically.

- Figure 5 is very helpful. Only minor suggestion is to increase the font sizes.

Areas for Improvement

To summarize the areas of improvement from my review:

- Some of the text in figures is small and can be made bigger. For example, the numbers in Figure 2, the cells in Figure 5, and the text in Figure 6.

- I think there are open questions about the ecological validity of the study that can be addressed in the method section. Is this task too simple since it only takes a few minutes to complete? Are the notebooks representative of realistic notebooks? What exactly were the post-study questions?

Suggestions for Online Appendix Content:  

Most ACM journal papers are researcher-oriented. Is this paper of potential interest to developers and engineers?: Maybe

Please help ACM create a more efficient time-to-publication process: Using your best judgment, what amount of copy editing do you think this paper needs?: Light

**
Referee: 2

Recommendation: Needs Minor Revision

Comments:
(There are no comments.)

Additional Questions:
The Review:  
This paper discusses documentation strategies in Computational Notebooks. It presents a study of 80 high-quality computational notebook, deriving a categorization of documentation. Based on this study, the authors propose Themisto a system facilitating the creation of explanation / markdown cells in computational notebooks. A preliminary study with  data scientists shows that they can create explanations faster with Themisto.

The paper is a solid contribution to the existing scholarship on computational notebooks. It provides an interesting classification of markdown cells, and a system that appears to be promising. Given some minor revisions addressed it would be a great TOCHI paper.

### Framing and positioning of the work

As an general note, I was surprised by the discrepancy between the positioning around human-AI collaboration, and the actual contribution of the paper. The topic is quite popular at the moment, but there is no human-AI _collaboration_ in Themisto. A prompt/auto-filling that can be corrected by users can hardly fall in a collaboration category. I would suggest to scrap references to human-AI collaboration from the title/abstract, and be more precise about the forms of interactions between humans and systems that are at play.

In framing the work in the related work, Lau et al. paper could serve to structure 2.1 as it provides a good overview of the design space of notebooks. This could help position more clearly the work done with Themisto. Indeed improving explanations in computational notebooks can be done in many ways, and improve markdown cells is only one aspect. This would open up the discussion to other "intelligent" strategies that could be put into place to support explanations in notebooks. Many strategies interact with markdown comments: breaking-down cells could help with more straightforward comments, supporting cell re-ordering could help with better headers/structrue, facilitating cell folding could help surface important markdown cells (see Rule et al. CSCW'18), or support for history (Kery et al.) and branching (Wood et al.) would also help create simpler or richer narratives.

To rephrase the critique, the paper does an excellent job of addressing commenting as it currently exists in Jupyter Notebook. But this is only one possibility in a much broader design space. While the work is solid, the initial framing and the discussion would benefit from engaging more deeply with the possibilities of improving narration in notebooks, and how intelligent strategies could be used not only for md cells.

In addition to this, I think that Woods et al. "Design Exposition with Literate Visualization" who also be worth discussing as it proposes interesting profiles on rather than a "one size fits all" approach to how literate programming should be.

### Formative Study

The formative study is nicely conducted and an excellent contribution to the literature.

My only comment relates to the naming of categories:
1. I did not understand if TODO relates to announcing the structure of an upcoming analysis (present and already coded in the notebook), or if it related to plan for later implementation. Given the absence of structure category it may be better to rename as such. Indeed in messier/less popular notebooks than the ones in the corpus cells with tasks to adress later will likely be present.
2. I did not understand the precise distinction between reason and education. I understand that education is more about background knowledge, but it seems to strongly relate to reason. Maybe background explanation/knowledge would be better than education. Such statement can be useful reminders for later notebook revisions rather than "educational" per see.

Overall this hints at a limit of the corpus which should be ackowledged. By focusing the analysis on "super clean" notebooks, the authors may have left out some varieties of markdown cells that exist in messy notebooks that would benefit from "intelligent" support.

Table 2 could be complemented by a plot showing the distribution of markdown cells.

A short discussion about the treatment of comments in the code rather than in markdown cells would be welcome (beside transforming the first line of comments into md) -> Were there many comments ? Are they just commented code or extra explanations?


### Themisto
The presentation of the system is clear and nicely readable for a non-expert. I am not specialist of the deep-learning so cannot say if enough information is provided to replicate the work.

Two elements could be further clarified :
- how much does the notebooks used for the training shape the quality/relevance of the ouputs? What were the competitions used?
- how was the dataset assembled and to what extent outputs differ from inputs (i.e., would some output infringe on copyright ?). Given the recent Github copilot controversy, it would be useful to have clarifications on the broader principles described.

### Experiment
The experimental set-up seeks to reproduce in a controlled way a commenting activity. There are inherent limits to the exercise, but this would be the topic of another paper investigation how Themisto is useful in the wild. The existing experiment does a decent job of testing the value of Themisto features on very simple notebooks.

One significant element remaining unclear is whether the two different data-science problems are in some ways related to the training data, as this would likely influence the results.  

### Discussion
This is the place to engage much more deeply with (1) human-ai collaboration for documentation, and (2) using your approach to support better documentation beyond the generation of markdown.

As nicely noted by one participant and discussed in 6.3.3 literate programming recommends writing comments before code. But more than that, the idea is of an incremental creation of code and explanations. The discussion could reflect on this dual dynamic where it is not code first or comments first but an incremental improvement that take place.

Beyond commenting suggestions, it seems that a tool like Themisto could also be used to generate code/comment smells, i.e., rather than suggesting fixes, flagging problematic areas to improve. Or providing positive feedback in case some cells are already well developed.

Related to this, is finally the question of evaluating / improving the comments in a more semantic fashion. Discussion on qualitative aspects of the code that are properly  generated by themisto and others that aren't would also be nice.

### Minor comments
- P2 L53/54 : prove the statement or tone it down. Some analysts do work on notebooks collaboratively, the
- P4 L199 : guidlines -> guidelines
- P5 L353 : practice is not the right term here.
- P5 L355 : stoped -> stopped
- P14 User Evaluation : were you expecting to see an effect of gender on the performance? if not, why report it?

Areas for Improvement

Identify aspects of the paper's presentation that need improvement including: *organization of the manuscript
*statements or passages that could be expressed more clearly and concisely
*figures that are redundant, difficult to understand, or missing
*incomplete or missing references, or citations that lack references
*changes that could make the paper more understandable to an international readership.  
You can also make any other recommendations that you think might be of use to the author(s). Please indicate which of your recommendations you consider to be conditions for acceptance, as opposed to optional suggestions.
 
Note that it is not necessary to comment on issues with formatting and layout, because these problems will be addressed by the copy editor and typesetter during final production.: see above

Suggestions for Online Appendix Content:  

The ACM Digital Library offers an online appendix feature, which allows authors to include additional content with their submissions beyond what can be included in the print article. This content may include additional text, videos, etc. If there is particular content that you believe should be included in the online appendix, please describe it here.:

Most ACM journal papers are researcher-oriented. Is this paper of potential interest to developers and engineers?: Yes

Please help ACM create a more efficient time-to-publication process: Using your best judgment, what amount of copy editing do you think this paper needs?: Light

**
Referee: 3

Recommendation: Needs Minor Revision

Comments:
(There are no comments.)

Additional Questions:
The Review:  
The contribution of this paper is an in-depth study of documentation practices in notebooks, followed by a novel system Themisto for supporting notebook documentation, followed by a solid HCI controlled user study of Themisto versus manual documentation. This paper gives excellent insights for tool builders in the HCI community on how automatic documentation support can be done in notebooks. Honestly, aside from a few nitpicks, I am a huge fan of this paper and find the work to be a journal-size contribution. It’s very rare to find an HCI paper that delivers in-depth highly rigorous qualitative research that directly informs in-depth rigorous system design, and then all comes together in an in-depth highly rigorous user study. The manuscript is a joy to read, and the attention to detail in research methods is a joy to see.

The research fills very timely gaps in terms of our *empirical* understanding of notebooks as explanatory communication narrative. In terms of technical novelty, Themisto uses a variety of familiar techniques for documentation generation, but combines them in new ways that very nicely tie automatic documentation generation with a careful understanding of what kinds of documentation notebook users want. The application of language models to documentation generation is timely and important, and Themisto is a very good HCI lens on that problem space.

My one concern with the storyline of the research is that the authors chose a beginner tutorial notebook corpus. The paper is currently missing a generalizability argument for this sample choice, which is a major issue. Why do we expect that beginner tutorial notebook documentation is representative of documentation in general data science notebooks used in industry or research? Are beginner-geared notebooks aspirational, some sort of ideal of what the authors believe documentation *should be*? I have much more minor line-level feedback, but this is the only crucial issue that rises to the level of a fix I consider conditional for acceptance.

Areas for Improvement

Line level feedback, optional but highly encouraged feedback:

- Good introduction. Off the bat I’m excited by this work and it sounds like a sensible approach that is very well motivated

- Ln 53 “besides, in real practice it is not common that multiple data scientists work on the same copy of a notebook and actively message each other.” I would tweak this to say “currently not common” as synchronous editing is a direction major notebook platforms like Jupyter are moving, and perhaps we’ll see more peer programming for data science in the future.

- Ln 10 Interesting. Kaggle is an excellent source… but are you going to get a sample bias that this is a platform focused on education and learning data science? I wonder if Kaggle notebooks may be more like tutorials than, for instance, notebooks published with papers?

- Ln 81 “Meanwhile, the quality of the documentation produced with Themisto are about the same as what data scientists produced on their own.” The phasing “about the same” sounds a wee bit casual and queues me to wonder how and if the authors measured documentation quality of automated versus manual documentation? Is this an empirical result or a general impression?

- Ln 173 “But those winning solutions are often not the most voted ones, as community members voted on readability and completeness of the computational narrative.” I don’t know if this characterization is entirely accurate. Do we know for sure that users are voting based on readability or completeness? A missing part of this characterization is that shared notebooks on Kaggle don’t all share the same purpose. Some are collaborative efforts shared during an active content [Tausczik & Wang 2017], some are tutorials written by the Kaggle platform, and some are computational narratives/tutorials/analysis walkthroughs written by members of the community **presumably because** even if you cannot win competitions, you can “win at” and gain ranking points and status, by writing popular notebooks ( see https://www.kaggle.com/progression). Tausczik & Wang found that notebooks written by higher-status members of the community or notebooks that are *more similar* to most other notebooks are more likely to get forked/edited by others. There may be a homogeneity affect going on in the sample here, that high ranked notebooks tend to follow certain style or technology conventions as other high ranked notebooks. I would like just a bit more detailed characterization of the Kaggle platform, because it really does affect what kind of data the authors are sampling in this study.
   - Relevant citation: Tausczik, Yla, and Ping Wang. "To share, or not to share? Community-level collaboration in open innovation contests." Proceedings of the ACM on Human-Computer Interaction 1, no. CSCW (2017): 1-23.

- Ln 180 “However, writing documentation itself is a time-consuming task. And that is why documentation practices in open source communities are widely perceived to be of low quality, due in part to low levels of intrinsic enjoyment for doing documentation work” Missing some of the key issues with software documentation: 1) documentation easily gets out-of-date and is expensive to keep updated over time, 2) it’s not clear how much documentation is needed, and 3) not all documentation is equally useful.
   - Relevant citation: Aghajani, Emad, Csaba Nagy, Olga Lucero Vega-Márquez, Mario Linares-Vásquez, Laura Moreno, Gabriele Bavota, and Michele Lanza. "Software documentation issues unveiled." In 2019 IEEE/ACM 41st International Conference on Software Engineering (ICSE), pp. 1199-1210. IEEE, 2019.

- Ln 251 “However, what types of documentation may be better suited for AI to do, and what works should the system leave to human data scientists? This is a design question that requires further exploration of the best practices for creating notebooks. Thus, we start this project with a formative study to fill this research gap.” Excellent ending to the related work and hook into the next section.

- Fig 2. Please label the red column and the blue column of plots, I had to read the figure caption several times to figure out red is Kaggle and blue is GitHub. Additionally, there are these tiny faint labels inside of the bottom 3 graphs that are redundant with the outside labels… maybe get rid of those. Finally, please make the x axis scale numbers a bit bigger for legibility, the same font size as the left labels ideally.

- Ln. 297  Why pick two beginners tutorial competitions? Why not take the most popular N notebooks from a random sample of the N most popular competitions or something like that? While it’s not a deal-breaker, I worry that this is a methodologically questionable choice. Beginner tutorial notebooks may not be representative of real data science work notebooks. Moreover, Rule et al.’s sample of notebooks is academic paper code, which may have very different characteristics than beginner tutorial notebooks? With these two samples, I’m not sure how to compare them. It seems like an apples to oranges comparison. Are Kaggle notebooks really better documented, as Fig 2. says, or are sample A and sample B meeting different communication goals for different audiences. How can you tell which one is better?

- Ln. 358 “Our analysis covered 4427 code cells and 3606 markdown cells within the 80 notebooks. Each notebook took around 1 hour to code as we coded the notebook at the cell level.” I have so much respect for how much time this analysis must have taken. The coding methods sound well done and reliable.

- Ln. 373 “We replicated tne notebook descriptive analysis” typo

- Ln. 381 “This result indicates that the 80 well-documented computational notebooks are better documented than general Github notebooks.” Again, I’m not sold that this is entirely true given the different audience and communication purposes of Sample A and Sample B. How do we know that sample A, which is more beginner tutorial oriented, doesn’t just contain more markdown because more needs to be explained for beginners? Sample B is notebooks with entire academic publications attached as documentation, so it makes some sense that they would be more brief? I like the comparative analysis and it’s interesting numbers, but I don’t think it is valid to make a value judgment better/worse given that A and B aren’t fully comparable.

- Table 2. Excellent table!

- Ln. 466 “External resources such as Uniform Resource Locators (URLs)” This is the first time I’ve seen what URL officially stands for! Maybe just say web links?

- “There is an ordinality in markdown cells that is aligned with the data science project’s lifecycle” Just a wording issue: I had to read this a few times to understand it. Is there a way to replace the word “ordinality”? I kept misreading it as “ordinarily”. Maybe just “This is an order to markdown cells…”

- “The notebook would be nice to have documentation with a problem overview at the beginning and a summary at the end.” Strange wording and not entirely grammatical?

- Ln. 479 “For the two barebone notebooks we used in the experiment, we always provide a problem overview as a markdown cell at the top of the notebook.” What experiment? Please don’t mention these notebooks here in the paper, as the experiment and its setup hasn’t been introduced yet.

- Fig 3. Nice Figure! Although it does trigger some sadness given the dataset choice.

- Fig. 4. Great visual.

- Ln. 607 “highly-voted notebooks from two popular Kaggle competitions” Which two? The same two as in Sample A? A different two? If different, please include a footnote link to the exact competitions. It’s helpful for the reader to look at as supplemental material to get a sense of how representative this data sample is.

- Ln. 616 “We also generate an AST for the source code input in step 2 with Python AST library7.” Were all collected notebooks in Python 3? I vaguely recall the Python 3 AST module does not like code from Python 2.

- Ln 617 “In step 3, we tokenize source code to a sequence of tokens with an input dictionary, and parse the AST nodes as a sequence of tokens with the same input dictionary.” I was following up until this point, but I really don’t understand step 3 or this sentence. A bit more detail to hold the reader’s hand through step 3 would be helpful! Tokenize like using Python’s tokenizer? How does one parse AST nodes as a sequence of tokens, if AST nodes are a data structure not plain text?

- Fig 5. Nice figure! I now see that “tokenize” in step 3 is *not* tokenize in the programming languages sense, but tokenize as in convert to an index in a dictionary. However, I still don’t fully see how the AST was tokenized: based on the node type name like “Assign?” Or something else?

- Fig 6. The code is way too small to read. I understand how hard it is to make figures showing code, but the 3 column layout here might not be possible. Perhaps 3 rows of A, B, C instead? Better extra-large code than tiny illegible code.

- Ln 674 “In the Appendix, we provide full code cells and model-generated outputs for the two experimental notebooks that we used in the user study.” I may have missed this detail, but I was looking for in this section: how long approximately does the model take to generate automatic documentation for a user? Milliseconds? Seconds? Minutes?This would be helpful to know.

- Ln 698 Missing at the end of this section: how does Themisto choose between the 3 approaches? Does it choose between them at this point as a prototype? Does Themisto suggest documentation for *every* cell, or are there cases in which it decides to leave a code cell as-is?

- Ln 724 “for the purpose of sharing those documented notebooks as tutorials” It’s a good thing here that the goal aligns well with the sample of notebooks from Kaggle. I am still wondering though about the framing of this paper: are beginner tutorial notebooks really what we are aiming for? I could certainly be convinced that tutorial notebooks are the epitome of a good computational narrative, but that argument is currently missing from the story. Beginner tutorial is a really specific flavor of documentation, but the paper is presenting this sample as generalizable and representative of all documentation? Or all documentation we should aim for? I’m unsure.

- Ln 800 Why have participants evaluate their own notebook rather than a peer grading situation or only the independent grader situation? A justification of this experiment design choice would be helpful.

- Ln 804 I’m a bit confused here: do the expert graders use the same rubric that participants used for themselves? How do these two grading schemes match up?

- Section 5.3 There are so many measures in this section (which is awesome by the way!) that it was very difficult to read. I would suggest breaking down section 5.3 into sub-sub-sections and also separate out by who collected what: A) what measures were from recordings B) what measures are from participants C) what measures are from independent graders (independent to the research team???) and D) what measures are from the research team coding sessions.

- Fig 7. There is one disagree or strongly disagree for each question, how intriguing. Was it all the same person who just happened to really hate the tool? A little context would be helpful in the caption.

- Ln 904 “The most interesting finding is that 41.24% markdown cells were co-created by Themisto and human participants together:” Thank you for bolding this, a statement like this is very helpful.

- Table 5. This table is brilliant.

- Ln 984 “Themisto generated the documentation with these three approaches, and asked participants if they like or dislike one particular approach.” I still am very confused on how Themisto picks between the 3 approaches. Does the user pick between the 3 in the UI?

- Ln 1038. “There was one participant who did not think Themisto could fit into his workflow:” Is this the participant who rated Themisto negatively???

- Ln 1185 “6.3.3 Inverting Themisto – Automatic Code Generation from Documentation.” Isn’t this just the entire research field of program synthesis? :)

- Results:  I’m yearning to see some examples of the co-created documentation. What did the machine generate and what did the human add to it or how did they edit it? Even just an illustrative figure or table showing some examples would be excellent.

Suggestions for Online Appendix Content:  

The ACM Digital Library offers an online appendix feature, which allows authors to include additional content with their submissions beyond what can be included in the print article. This content may include additional text, videos, etc. If there is particular content that you believe should be included in the online appendix, please describe it here.: It would be fantastic for the authors to include a printout of the notebooks generated by participants in the study, just to see what the generated documentation looked like.

Most ACM journal papers are researcher-oriented. Is this paper of potential interest to developers and engineers?: Maybe

Please help ACM create a more efficient time-to-publication process: Using your best judgment, what amount of copy editing do you think this paper needs?: None

==> review/summary_of_changes.tex <==
We thank all the reviewers for your thoughtful and comprehensive feedback. We used your feedback to revise and improve our submission, as we explain the details below. We highlighted all the changes in red in the revised manuscript.

We first addressed the two critical issues summarized in the meta-review.

1. Address the Ecological Validity of the Study (R1, R2, and R3); Discuss the Limitation of the Kaggle Corpus (R3)
We addressed the concerns and questions about the validity of the study in sections 5.2 and 5.3. We expanded the limitation section 6.4 to discuss the limitation of studying the Kaggle Corpus in the formative study.

2. Change the Framing around Human-AI Collaboration (R2)
We revised the framing around Human-AI collaboration as R2 suggested in the abstract and introduction (section 1). We removed the references to Human-AI collaboration, and engaged the framing more deeply with the possibilities of improving narration in notebooks. We only included Human-AI collaboration as a discussion theme.

In addition, we revised the other points based on reviewers' suggestions.

- We elaborated on the long-term impact of Themisto on users' performance in the discussion section 6.2. (R1)
- We included visual components in Table 4 (now Table 5). (R1)
- We updated Figure 7 (now Figure 6) to include the complete results from the post-task questionnaire. (R1)
- We clarified the naming categories in the formative study (Table 1). (R2)
- We clarified some implementation details in sections 4.2 and 4.3. (R2, R3)
- We expanded section 6 to deepen the discussions. (R2)
- We revised the related work section (section 2) to include additional references. (R3)
- We updated Figure 2 and Figure 6 (now Table 3) to improve the presentation. (R3)
- We added examples of co-created documentation in the appendix. (R3)

==> sections/table3.tex <==
% Please import the tabmint package
% \usepackage[finalizecache,cachedir=.]{minted}

% \setminted[c]{
%     breaklines,
%     fontsize=\footnotesize,
%     }
% \makeatletter
% \newenvironment{tabminted}{
%     \let\FV@ListVSpace\relax  
%     \minted
% }{%
%     \endminted
%     \unskip   
%     \aftergroup\@tabmintedend
% }
% \newcommand*{\tabminted@finalstrut}[1]{%
%     \ifdim\prevdepth>0pt
%         \ifdim\dp#1>\prevdepth
%             \vskip\dimexpr(\dp#1)-\prevdepth\relax
%         \fi
%     \else
%         \vskip\dimexpr(\dp#1)\relax
%     \fi
% }
% \newcommand*{\@tabmintedend}{%
%     \let\@finalstrut\tabminted@finalstrut
% }
% \makeatother

\begin{table}[t!]
\small
\centering
\caption{\revision{Example output from the model. (Example A) The generated text well describes the code. (Example B) The generated text vaguely describes the code. (Example C) The generated text is poorly readable, but still captures the keywords of the descriptions.}}
\label{tab:example_output}
\begin{tabular}{p{2cm}p{7cm}p{5cm}} 
 \toprule
 \textbf{Example} & \textbf{Code Cell} & \textbf{Output From the Model}\\
 \midrule
 Example A &
\begin{tabminted}{python}
train = pd.read_csv('./house-input/train.csv')
test = pd.read_csv('./house-input/test.csv')
\end{tabminted}
& Read the data
\\
\hline
Example B &
\begin{tabminted}{python}
all_data = pd.get_dummies(all_data)
\end{tabminted} 
& Convert all the data\\
\hline
Example C &
\begin{tabminted}{python}
pred = Tree_model.predict(x_test)
pred = pd.DataFrame(pred)
pred.columns = ["ConfirmedCases_prediction"]
\end{tabminted}
& Predicate to use a predicct function for tests \\
\bottomrule
\end{tabular}
\end{table}

==> sections/table7.tex <==
% Please import the tabmint package
% \usepackage[finalizecache,cachedir=.]{minted}

% \setminted[c]{
%     breaklines,
%     fontsize=\footnotesize,
%     }
% \makeatletter
% \newenvironment{tabminted}{
%     \let\FV@ListVSpace\relax  
%     \minted
% }{%
%     \endminted
%     \unskip   
%     \aftergroup\@tabmintedend
% }
% \newcommand*{\tabminted@finalstrut}[1]{%
%     \ifdim\prevdepth>0pt
%         \ifdim\dp#1>\prevdepth
%             \vskip\dimexpr(\dp#1)-\prevdepth\relax
%         \fi
%     \else
%         \vskip\dimexpr(\dp#1)\relax
%     \fi
% }
% \newcommand*{\@tabmintedend}{%
%     \let\@finalstrut\tabminted@finalstrut
% }
% \makeatother

 \begin{landscape}
\section{Example of Documentation Generation in Themisto}
\begin{table}[h]
\small
\centering
\caption{\revision{Example notebook (House Prediction), documentation generation in Themisto, and user submitted documentation (T - Markdown Cells Created by Themisto Only, C - Markdown Ceells Co-created by Humans and Themisto, H - Markdown Cells Created by Humans Only).}}
\label{tab:notebook-house}
\begin{tabular}{p{5.5cm}p{2cm}p{3.5cm}p{2cm}p{3.8cm}} 
 \toprule
 \textbf{Source Code} & \textbf{DL-Based} & \textbf{Query-Based} & \textbf{Prompt-Based} & \textbf{P2}\\
 \midrule
\begin{tabminted}{python}
import pandas as pd
import numpy as np
from sklearn.linear_model import LassoCV
from sklearn.model_selection 
    import cross_val_score
\end{tabminted}
& Importing libraries 
& Pandas is for data manipulation and analysis; NumPy is a library for ... 
& This code cell is for \_ \_ \_ \_ \_ 
& Importing libraries (T)\\
\midrule
\begin{tabminted}{python}
train = pd.read_csv('train.csv')
test = pd.read_csv('test.csv')    
\end{tabminted}
& Read the data
& Read a comma-separated values (csv) file into DataFrame; Return the first 5 rows.
& This code cell is for \_ \_ \_ \_ \_ 
& Read the data (T)\\
\midrule
\begin{tabminted}{python}
train.head()
\end{tabminted}
& Let's see the values
& Return the first 5 rows
& The table shows \_ \_ \_ \_ \_ 
& Return the first 5 rows. (defValue=5) (C)\\
\midrule
\begin{tabminted}{python}
all_data = pd.concat((
train.loc[:,'SubClass':'SaleCond'],
test.loc[:,'SubClass':'SaleCond'])) 
\end{tabminted}
& A generator for feature
& Concatenate pandas objects along a particular axis with optional set logic along the other axes.
& This code cell is for \_ \_ \_ \_ \_ 
& Concat train and test col "SaleCondition" (C)\\
\midrule
\begin{tabminted}{python}
all_data = pd.get_dummies(all_data)
\end{tabminted}
& Convert all the data
& Convert categorical variable into dummy/indicator variables
& This code cell is for \_ \_ \_ \_ \_ 
& Convert categorical variable into dummy/indicator variables. (T)\\
\midrule
\begin{tabminted}{python}
all_data = all_data
    .fillna(all_data.mean())
 \end{tabminted}
 & Check the missing values
 & Fill NA/NaN values using the specified method
 & This code cell is for \_ \_ \_ \_ \_ 
 & \\
 \midrule
\begin{tabminted}{python}
X_train = all_data[:train.shape[0]]
X_test = all_data[train.shape[0]:]
y = train.SalePrice
 \end{tabminted}
 & Create the target and the test data
 & Slice string
 & This code cell is for \_ \_ \_ \_ \_ 
 & \\
 \midrule
\begin{tabminted}{python}
model_lasso = LassoCV(
    alphas = [1, 0.1, 0.001, 0.0005])
    .fit(X_train, y)
 \end{tabminted}
 & Model
 & Lasso linear model with iterative fitting along a regularization path.
 & This code cell is for \_ \_ \_ \_ \_ 
 & Fit regression model (H)\\
 \midrule
\begin{tabminted}{python}
def rmse_cv(model):
    rmse= np.sqrt(-cross_val_score(
        model, X_train, y, scoring=
        "neg_mean_squared_error", cv = 5))
    return(rmse)
rmse_cv(model_lasso).mean()
 \end{tabminted}
 & A simple example model with the lasso
 & Evaluate a score by cross-validation
 & The result indicates that \_ \_ \_ \_ \_ 
 & Define score function and evaluate (H)\\
 \bottomrule
\end{tabular}
\end{table}
\end{landscape}

==> sections/table8.tex <==
% Please import the tabmint package
% \usepackage[finalizecache,cachedir=.]{minted}

% \setminted[c]{
%     breaklines,
%     fontsize=\footnotesize,
%     }
% \makeatletter
% \newenvironment{tabminted}{
%     \let\FV@ListVSpace\relax  
%     \minted
% }{%
%     \endminted
%     \unskip   
%     \aftergroup\@tabmintedend
% }
% \newcommand*{\tabminted@finalstrut}[1]{%
%     \ifdim\prevdepth>0pt
%         \ifdim\dp#1>\prevdepth
%             \vskip\dimexpr(\dp#1)-\prevdepth\relax
%         \fi
%     \else
%         \vskip\dimexpr(\dp#1)\relax
%     \fi
% }
% \newcommand*{\@tabmintedend}{%
%     \let\@finalstrut\tabminted@finalstrut
% }
% \makeatother

\begin{landscape}
\begin{table}[ht!]
\small
\centering
\caption{\revision{Example notebook (Covid Prediction), documentation generation in Themisto, and user submitted documentation (T - Markdown Cells Created by Themisto Only, C - Markdown Ceells Co-created by Humans and Themisto, H - Markdown Cells Created by Humans Only).}}
\label{tab:notebook-covid}
\begin{tabular}{p{5.5cm}p{2cm}p{3.5cm}p{2cm}p{3.8cm}} 
 \toprule
 \textbf{Source Code} & \textbf{DL-Based} & \textbf{Query-Based} & \textbf{Prompt-Based} & \textbf{P5}\\
 \midrule
\begin{tabminted}{python}
import numpy as np
import pandas as pd
from sklearn.ensemble 
    import RandomForestClassifier
\end{tabminted}
& Importing libraries 
& Pandas is for data manipulation and analysis; NumPy is a library for ... 
& This code cell is for \_ \_ \_ \_ \_ 
& Importing libraries (T)\\
\midrule
\begin{tabminted}{python}
train = pd.read_csv("train.csv")
test = pd.read_csv("test.csv")
train.head()    
\end{tabminted}
& Read the data
& Read a comma-separated values (csv) file into DataFrame; Return the first 5 rows.
& The table shows \_ \_ \_ \_ \_ 
& Read and sanity check the data (C)\\
\midrule
\begin{tabminted}{python}
train.describe()
\end{tabminted}
& Let's see the values
& Generate descriptive statistics. Descriptive statistics include ...
& The table shows \_ \_ \_ \_ \_ 
& \\
\midrule
\begin{tabminted}{python}
train["Date"] = train["Date"]
    .apply(lambda x: x.replace("-",""))
train["Date"] = train["Date"]
    .astype(int)
train.head() 
\end{tabminted}
& Convert all the data
& Replace a specified phrase with another specified phrase
& The table shows \_ \_ \_ \_ \_ 
& Preprocess the data (C)\\
\midrule
\begin{tabminted}{python}
train.isnull().sum()
\end{tabminted}
& Check the missing values
& Detect missing values for an array-like object
& The result indicates that \_ \_ \_ \_ \_ 
& Check the missing values (T)\\
\midrule
\begin{tabminted}{python}
test["Date"] = test["Date"]
    .apply(lambda x: x.replace("-",""))
test["Date"]  = test["Date"]
    .astype(int) \end{tabminted}
& Convert all the data
& Replace a specified phrase with another specified phrase
 & This code cell is for \_ \_ \_ \_ \_ 
 & Preprocess the date column (C)\\
 \midrule
\begin{tabminted}{python}
x = train[['Lat', 'Long', 'Date']]
y = train[['ConfirmedCases']]
x_test = test[['Lat', 'Long', 'Date']]
\end{tabminted}
 & Create the target and the test data
 & Select subsets of data
 & This code cell is for \_ \_ \_ \_ \_ 
 & Create the train/test data and the target (C)\\
 \midrule
\begin{tabminted}{python}
Tree_model = RandomForestClassifier(
    max_depth=200, 
    random_state=0)
Tree_model.fit(x,y)
 \end{tabminted}
 & Model
 & A random forest is a meta estimator that fits a number of decision tree classifiers on ...
 & This code cell is for \_ \_ \_ \_ \_ 
  & Define and configure the model

A random forest is a meta ... We also train the model with `.fit()` (C)\\
 \midrule
\begin{tabminted}{python}
pred = Tree_model.predict(x_test)
pred = pd.DataFrame(pred)
pred.columns = 
    ["ConfirmedCases_prediction"]
 \end{tabminted}
 & Predicate to use a predicate function for tests
 & A random forest is a meta estimator that fits a number of decision tree classifiers on ...
 & This code cell is for \_ \_ \_ \_ \_ 
 & Run the model to generate predictions on the test data and store them as a `DataFrame`(H) \\
 \bottomrule
\vspace{1mm}
\end{tabular}
\end{table}
\end{landscape}
